AutoHOOT: Automatic High-Order Optimization for Tensors

High-order optimization methods, including Newton's method and its variants as well as alternating minimization methods, dominate the optimization algorithms for tensor decompositions and tensor networks. These tensor methods are used for data analysis and simulation of quantum systems. In this work, we introduce AutoHOOT, the first automatic differentiation (AD) framework targeting at high-order optimization for tensor computations. AutoHOOT takes input tensor computation expressions and generates optimized derivative expressions. In particular, AutoHOOT contains a new explicit Jacobian / Hessian expression generation kernel whose outputs maintain the input tensors' granularity and are easy to optimize. The expressions are then optimized by both the traditional compiler optimization techniques and specific tensor algebra transformations. Experimental results show that AutoHOOT achieves competitive CPU and GPU performance for both tensor decomposition and tensor network applications compared to existing AD software and other tensor computation libraries with manually written kernels. The tensor methods generated by AutoHOOT are also well-parallelizable, and we demonstrate good scalability on a distributed memory supercomputer.

==> notation.tex <==

For vectors, bold lowercase Roman letters are used, e.g., $\vcr{x}$. For matrices, bold uppercase Roman letters are used, e.g., $\mat{X}$. For tensors, bold calligraphic uppercase Roman letters are used, e.g., $\tsr{X}$. An order $N$ tensor corresponds to an $N$-dimensional array with dimensions $s_1\times \cdots \times s_N$. 

Elements of vectors, matrices, and tensors are denoted in parentheses, e.g., $\vcr{x}(i)$ denotes the $i$th entry of a vector $\vcr{x}$, $\mat{X}(i,j)$ denotes the $(i,j)$th element of a matrix $\mat{X}$, and $\tsr{X}(i,j,k,l)$ denotes the $(i,j,k,l)$th element of an order 4 tensor $\tsr{X}$. Elements of a function output are denoted by subscripts. Matricization is the process of unfolding a tensor into a matrix. Given a tensor $\tsr{X}$ the mode-$n$ matricized version is denoted by $\mat{X}_{(n)}\in \R^{s_n\times K}$ where $K=\prod_{m=1,m\neq n}^N s_m$. We generalize this matricization definition, so that $\mat{X}_{[i:j]}$ means that the dimensions from the $i$th index to the $j$th index are unfolded to the column dimension of the matrix, and all the other dimensions are unfolded to the row dimension of the matrix.

For a scalar output function $y=f(\vcr{a}_1, \ldots, \vcr{a}_N)$, We use the $\vcr{g}^{[f]}_{[\vcr{a}_i]}$ and $\mat{H}^{[f]}_{[\vcr{a}_i]}$ to denote the gradient vector and Hessian matrix of $f$ w.r.t the input vectors $\vcr{a}_i$. When the inputs are tensors, the gradient and the Hessian will also be a tensor and denote $\tsr{G}^{[f]}_{[\tsr{A}_i]}$ and $\tsr{H}^{[f]}_{[\tsr{A}_i]}$. For a function non-scalar output $\vcr{y} = f(\vcr{a}_1, \ldots, \vcr{a}_N)$, We use $\mat{J}^{[f]}_{[\vcr{a}_i]}$ to denote the Jacobian matrix of the function $f$ w.r.t one of the input vectors $\vcr{a}_i$. The shape of the Jacobian matrix will be $\R^{|\vcr{y}|\times|\vcr{a}_i|}$. If $\tsr{Y}$ is an output tensor with size $\R^{s_1\times \ldots \times s_M}$, and $\tsr{A}_i$ is an input tensor with size $\R^{r_1\times \ldots\times r_K}$, then the Jacobian will be a tensor denoting $\tsr{J}^{[f]}_{[\tsr{A}_i]}$, and has size $\R^{s_1\times \ldots\times s_M\times r_1\times\ldots\times r_K}$. 

We also define generalized Vector-Jacobian Product (VJP), Jacobian-Vector Product (JVP) and Hessian-Vector Product (HVP). 
When both Jacobian and Hessian are matrices, these are matrix multiplication operations. 
When Jacobian and Hessian are both tensors defined above, these are tensor contractions, whose results are the same as unfolding the tensors into matrices and perform the matrix-vector product.

For a tensor $\tsr{A}\in\R^{s_1\times \ldots \times s_N}$, we define its norm $\|\tsr{A}\|$ as the square root of its inner product. We define the norm $\|\tsr{A}\|_{\tsr{X}}=\sqrt{\vcr{a}^T_{[1:N]} \mat{X}_{[1:N]}\vcr{a}_{[1:N]}}$ if $\tsr{X}\in\R^{s_1\times \ldots \times s_N\times s_1\times \ldots \times s_N}$ and $\mat{X}_{[1:N]}$ is positive semi-definite. 

The computations in AutoHOOT are described by \textit{computational graphs}, which are directed graphs revealing the data dependency between different operations. Each \textit{node} can be source, intermediate or sink. Source/Sink nodes are inputs/outputs of the graph. Sink and intermediate nodes can be any mathematical computation, while input nodes are fed by the user or constants.  An \textit{edge} connecting two nodes represents the data dependency between them. An example of a computational graph is shown in Figure~\ref{fig:graph_example}, which represents the addition of two Einsum results. Here $\tsr{A}, \tsr{B}, \tsr{C}$ are source nodes, the Einsum node is the sink. We typically refer the with its type, e.g Einsum node, which represents the tensor computations based on the Einstein summation convention.
\textit{Einsum graph} is defined as a graph of nodes where all the nodes except sources must be Einsum nodes. 
\textit{Einsum tree} is defined as a tree of nodes where all the nodes except leaves must be Einsum nodes. 

\begin{figure}[t]
\centering
\includegraphics[width=1.3in]{pic/graph_example.pdf}
\caption{An example of a computational graph. We use green nodes to denote input variables, purple nodes to denote output nodes, and blue nodes to denote intermediate or constant nodes.}
\label{fig:graph_example}
\end{figure}
